Educators' Perceptions of Large Language Models as Tutors: Comparing Human and AI Tutors in a Blind Text-only Setting

The rapid development of Large Language Models (LLMs) opens up the possibility of using them as personal tutors. This has led to the development of several intelligent tutoring systems and learning assistants that use LLMs as back-ends with various degrees of engineering. In this study, we seek to compare human tutors with LLM tutors in terms of engagement, empathy, scaffolding, and conciseness. We ask human tutors to annotate and compare the performance of an LLM tutor with that of a human tutor in teaching grade-school math word problems on these qualities. We find that annotators with teaching experience perceive LLMs as showing higher performance than human tutors in all 4 metrics. The biggest advantage is in empathy, where 80% of our annotators prefer the LLM tutor more often than the human tutors. Our study paints a positive picture of LLMs as tutors and indicates that these models can be used to reduce the load on human teachers in the future.

==> tables/macdonald_corr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\resizebox{\linewidth}{!}{\begin{tabular}{|c|c|c|c|}
\hline
\rowcolor[HTML]{212121} 
{\color[HTML]{FFFFFF} Metric Name}                                                                        & {\color[HTML]{FFFFFF} \begin{tabular}[c]{@{}c@{}}Applicable to \\ Our Setting\end{tabular}} & {\color[HTML]{FFFFFF} Maps To} & {\color[HTML]{FFFFFF} Comments}                                                                                                    \\ \hline
Promote independence in learning                                                                          & Yes                                                                                         & Scaffolding                    & This mapping is almost exact                                                                                                       \\ \hline
Personalize instruction                                                                                   & Partially                                                                                   & Engagement                     & \begin{tabular}[c]{@{}c@{}}There is short term and long term \\ personalisation, only the former \\ is evaluable here\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}Facilitate tutee insights into \\ learning and learning processes\end{tabular} & Yes                                                                                         & Scaffolding                    & This mapping is almost exact                                                                                                       \\ \hline
\begin{tabular}[c]{@{}c@{}}Provide a student perspective on\\  learning and school success\end{tabular}   & No                                                                                          & N/A                            & This is an administrative goal                                                                                                     \\ \hline
Respect individual differences                                                                            & Partially                                                                                   & Empathy                        & \begin{tabular}[c]{@{}c@{}}We adapt only to academic \\ differences, not cultural differences\end{tabular}                         \\ \hline
Follow a Job Description                                                                                  & No                                                                                          & N/A                            & This is an administrative goal                                                                                                     \\ \hline
\end{tabular}}
\caption{Correspondence between MacDonalds's\cite{macdonald2000master} metrics and our metrics. We encourage readers to go over the first chapter of MacDonald's Book for his definition of the metrics}
\label{tab:macdonald_corr}
\end{table}

==> tables/maurya_corr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\resizebox{\linewidth}{!}{\begin{tabular}{|c|c|c|c|}
\hline
\rowcolor[HTML]{212121} 
{\color[HTML]{FFFFFF} Metric Name} & {\color[HTML]{FFFFFF} \begin{tabular}[c]{@{}c@{}}Applicable to \\Our Setting\end{tabular}} & {\color[HTML]{FFFFFF} Corresponding Metric} & {\color[HTML]{FFFFFF} Comments}                                                 \\ \hline
Mistake Identification             & Yes                                                                                                 & Scaffolding/Engagement                      &                                                                                 \\
Mistake Location                   & Yes                                                                                                 & Scaffolding/Engagement                      & \multirow{-2}{*}{These are yes/no questions, not suitable for ranking} \\\hline
Revealing The Answer               & Partially                                                                                               & Scaffolding/Engagement                      & Revealing often happens towards the end of conversations                        \\\hline
Providing Guidance                 & Yes                                                                                                 & Scaffolding                                 & This mapping is almost exact                                                    \\\hline
Actionability                      & Yes                                                                                                 & Engagement                                  &                                                                                 \\\hline
Coherence                          & Yes                                                                                                 & Engagement                                  &                                                                                 \\\hline
Tutor tone                         & Yes                                                                                                 & Empathy                                     &                                                                                 \\\hline
Human Likeness                     & Yes                                                                                                 & Empathy                                     & It is not clear if we should be comparing this when one side is human           \\ \hline
\end{tabular}}
\caption{Correspondence between Maurya et. al.'s metrics and our metrics}
\label{tab:maurya_corr}
\end{table}
